Autoencoders for discovering manifold dimension and coordinates in data from complex dynamical systems

While many phenomena in physics and engineering are formally high-dimensional, their long-time dynamics often live on a lower-dimensional manifold. The present work introduces an autoencoder framework that combines implicit regularization with internal linear layers and $L_2$ regularization (weight decay) to automatically estimate the underlying dimensionality of a data set, produce an orthogonal manifold coordinate system, and provide the mapping functions between the ambient space and manifold space, allowing for out-of-sample projections. We validate our framework's ability to estimate the manifold dimension for a series of datasets from dynamical systems of varying complexities and compare to other state-of-the-art estimators. We analyze the training dynamics of the network to glean insight into the mechanism of low-rank learning and find that collectively each of the implicit regularizing layers compound the low-rank representation and even self-correct during training. Analysis of gradient descent dynamics for this architecture in the linear case reveals the role of the internal linear layers in leading to faster decay of a "collective weight variable" incorporating all layers, and the role of weight decay in breaking degeneracies and thus driving convergence along directions in which no decay would occur in its absence. We show that this framework can be naturally extended for applications of state-space modeling and forecasting by generating a data-driven dynamic model of a spatiotemporally chaotic partial differential equation using only the manifold coordinates. Finally, we demonstrate that our framework is robust to hyperparameter choices.

==> ProblemSetUp.tex <==
\begin{singlespace}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.35\textwidth]{AE_vanilla}
		\caption[]{Typical feed-forward deep autoencoder architecture.}
		\label{fig:AE_vanilla}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.90\textwidth]{Schematic_ImplicitWD}
		\caption[]{Our Implicit $\lambda$ Regularized deep autoencoder framework}
		\label{fig:AE_IRLamda}
	\end{center}
\end{figure}

Our proposed framework uses an autoencoder framework. Autoencoders are composed of two subnetworks, the encoder and decoder, which are connected by a latent hidden layer. For dimensionality reduction problems, this latent hidden layer is often a size-limiting bottleneck that explicitly restricts the number of degrees of freedom that the input data can be represented by. This forces the encoder network, $z=\mathcal{E}(u;\theta_{E})$, to compressed the input data, $u\in\mathbb{R}^{d_n}$, into a compact representation, $z\in\mathbb{R}^{d_z}$, where $d_n > d_z$. The decoder, $\tilde{u}=\mathbb{D}(z;\theta_{D})$, is tasked with the inverse task of learning to reconstruct the input, $\tilde{u}\in\mathbb{R}^{d_n}$, from the compressed representation, $z$. The autoencoder is trained to minimize the mean squared reconstruction loss (MSE),

\begin{equation}
\mathcal{L}(u;\theta_E,\theta_D) = \langle ||u-\mathcal{D}(\mathcal{E}(u;\theta_E);\theta_{D})||^2 \rangle
\label{eq:AE_loss}
\end{equation}

 Here we use the $L_2$ norm ($p=2$) and $\langle\cdot\rangle$ is the average over a training batch. We then deviate from the typical vanilla/diabolo networks by adding an additional linear network, $\mathcal{W}(\cdot;\theta_W)$, between the encoder network and decoder. $\mathcal{W}(\cdot;\theta_W)$ is composed of $n$ trainable linear weight matrices (i.e. linear layers) of size $d_z\times d_z$ in series, similar to that done by \citep{Jing2020}. Although this series of linear blocks add additional training parameters compared to a vanilla autoencoder, it does not give the network any additional expressivity, as linear layers in series have the same expressivity as a single linear layer. Thus, the effective capacity between the two networks are identical. We train the framework under the autoassociation task with the addition of weight-decay,

 \begin{equation}
\mathcal{L}(u;\theta_E,\theta_W,\theta_D) = \langle ||u-\mathcal{D}(\mathcal{W}(\mathcal{E}(u;\theta_E);\theta_{W});\theta_{D})||^2 \rangle + \dfrac{\lambda}{2}  {\left\lVert \theta \right\rVert}_p^2
\label{eq:our_loss}
\end{equation}

Here we contrast our framework from typical vanilla autoencoders tasked with finding minimal or low-dimensional representations with two distinctions. First, rather than parametrically sweep $d_z$, as is usually done with vanilla autoencoders, we instead guess a single $d_z > d_m$. We rely on implicit regularization and weight-decay to drive the latent space to an approximately minimal rank representation while relying on the autoassociation task to prevent information loss. 

Once the regularized network is trained, we perform singular value decomposition on the covariance matrix of the latent space $z$. Here, the number of significant singular values of this spectra gives an estimate of $d_m$, as each significant value represents a necessary coordinate in representing the original data. The corresponding significant singular vectors also allow us to map from $z$ to $h$, isolating the ``manifold'' coordinate representation with an orthogonal and approximately lossless transformation.




\end{singlespace}
\newpage

==> Results.tex <==
\begin{singlespace}

\begin{itemize}
	\setlength\itemsep{0pt}
	\setlength{\parskip}{0pt}
	\item introduce baseline test--linearly embedded data
	\item introduce chaotic manifold nonlinearly embedded in higher dimension
	\item extend to infinite dimensional PDEs
	\item mention comparison to predecessor data sets (MNIST, CelebA)
	\item discuss mechanism (SV evolution through the model, SV evolution through training)
	\item discuss parameter influence: $c$, $L$
	\item discuss failure points of method
	\item demonstrate forecasting framework
	\item Consider t-sne, UMAP \KZ{these require inputing $d_h$}
	\item consider Diffusion map
	\item \MDG{compare/comment on Wang and Guet paper with penalty on off-diagonal elements of covariance}
	\item \MDG{comment on paper Vinuesa cites -- variational beta autoencoder?}
	\item \MDG{\sout{combine with clustering -- should get the same dimension estimate for each cluster -- apply to Daniel/Andrews heteroclinic KSE example?}}
	\item \MDG{would like to see a more complex charts example -- what's wrong with Daniel's bursting example? }
	\item \MDG{\sout{KSE at various $L$ to look at scaling of $d_M$ with $L$}}
	\item \MDG{another method to point out/consider -- locally linear embedding (LLE)}
\end{itemize}
\newpage
\subsection{Manifold Dimension Estimates: Example Systems}
We now investigate our method applied to a zoo of data sets of increasing complexity. These systems range from linearly embedded manifolds in finite-dimensional ambient spaces to nonlinearly embedded manifolds in infinite-dimensional ambient spaces.

\subsubsection{Finite dimensional system linearly embedded in a finite-dimensional ambient space}
We first benchmark our method against a simple finite dimensional system linearly embedded in a larger finite-dimensional ambient space i.e. an embedded hypercube dataset. This data set consists of 5 dimensional noise linearly embedded in an ambient space of 20 dimensions. Because this dataset exactly spans 5 orthogonal directions and is linearly embedded, Principal Component Analysis (PCA) is able to extract the dimensionality of the data, which can be identified via the singular value spectra. Shown in Fig.~\ref{fig:SV_OD} are the singular values obtained from PCA as well those obtained from the learned latent variables of our method and a standard AE. We show that PCA and our method parse out the linearly embedded data while a standard autoencoder does not. We further highlight here two important observations: 1) an autoencoder with weight decay alone is insufficient in learning a sparse representation 2) an autoencoder with implicit regularization alone, analogous to \citep{Jing2020} learns only an approximately sparse representation.

%Using Gram-Schmidt orthogonalization, a 20-dimensional orthonormal basis was obtained. The training dataset is comprised of 40,000 snapshots of 20 dimensional uniformly sampled noise vectors, each of which has had content in first 15 orthonormal directions removed such that the data only spans 5 orthogonal directions. This is done to ensure that the data ambiently resides in $\mathbb{R}^{20}$ while living on an underlying manifold of 5 dimensions. 

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.90\textwidth]{SV_EmbeddedNoise}
		\caption[]{Singular values of learned latent spaces for a $\mathbb{R}^{5}$ manifold linearly embedded in $\mathbb{R}^{20}$}
		\label{fig:SV_OD}
	\end{center}
\end{figure}

\subsubsection{Nonlinearly embedded finite-dimensional systems: The Archimedean Spiral Lorenz}

We now turn our attention to nonlinear finite dimensional dynamical systems with nonlinearly embedded manifolds. Specifically, we embed the nonlinear 3 dimensional Lorenz `63 system,
\begin{equation}
\begin{split}
\dot{x} &= \sigma(y-x) \\
\dot{y} &= x(\rho-z)-y \\
\dot{z} &= xy-\beta z
\end{split}
\label{eq:Lorenz}
\end{equation}

 in 4 dimensions by wrapping the Lorenz butterfly about the Archimedean spiral i.e. $[u_1, u_2, u_3, u_4] = [x, y, \alpha z \cos{(\alpha z)}, \alpha z \sin{(\alpha z)}] $, where $\alpha=0.2$. The evolution of the Archimedean Lorenz is defined as the follow,

\begin{equation}
\begin{split}
\dot{u_1} &= \sigma(u_2-u_1) \\
\dot{u_2} &= u_1 \left( \rho-\alpha^{-1} \sqrt{{u_3}^2+{u_4}^2} \right) - u_2 \\
\dot{u_3} &= \alpha^{-1} \left( u_1 u_2 - \beta \alpha^{-1} \sqrt{{u_3}^2+{u_4}^2} \right) \left(\cos{\left(\sqrt{u_4^2+{u_4}^2} \right)} - u_4\right)  \\
\dot{u_4} &= \alpha^{-1} \left( u_1 u_2 - \beta \alpha^{-1} \sqrt{{u_3}^2+{u_4}^2} \right) \left(\sin{\left(\sqrt{u_4^2+{u_4}^2} \right)} + u_3\right)  \\
\end{split}
\label{eq:ArchLorenz}
\end{equation}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.90\textwidth]{Data_ArchLorenz}
		\caption[]{Dynamics of the a) Lorenz `63 equation b) Archimedean Lorenz equation.}
		\label{fig:Data_ArchLorenz}
	\end{center}
\end{figure}

For the parameters $\sigma=10,\rho=28,\beta=8/3$,  the Lorenz '63 exhibits chaotic dynamics, which subsequently govern the Archimedean Lorenz. In other words, the underlying dynamics of this system live on a nonlinear 3 dimensional manifold that is nonlinearly embedded in a 4 dimensional ambient space. We show in Fig.~\ref{fig:SV_AL} that our method correctly isolates that this system can be minimally represented by 3 latent variables.  In contrast, the application of PCA fails to identify the underlying structure of the data. Here, the PCA spectra does not give a correct estimate of $d_m$ because inherently a linear method cannot minimally capture the nonlinearity/curvature of the manifold. Finally, a standard AE with $d_z > d_m$ also fails to automatically learn a minimal representation as it finds a full-rank latent space.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_AL_Combined}
		\caption[]{Singular values of learned latent spaces for the Archimedean Spiral Lorenz}
		\label{fig:SV_AL}
	\end{center}
\end{figure}

\subsubsection{Nonlinearly embedded infinite-dimensional systems: The Kuramoto-Sivashinsky Equation}

We now turn our attention to dissipate nonlinear systems that are formally ``infinite'' dimensional.
Here, we investigate the 1D periodic Kuramoto-Sivashinsky equation (KSE), which is a system that describes reaction-diffusion phenomena, flame-front velocity propagation, and fluid films. Under certain parameters, this system exhibits rich spatiotemporal chaotic dynamics which has made it a common proxy system for turbulent fluid flows. In order to analyze formally ``infinite'' dimensional systems, state snapshots will consist of sampled spatial collocation mesh points in the domain.

\begin{equation}
\frac{\partial v}{\partial t} = -v\frac{\partial v}{\partial x} -\frac{\partial^2 v}{\partial x^2} -\frac{\partial^4 v}{\partial x^4}
\label{eq:KSE}
\end{equation}

We apply our framework to extract the dimension of the underlying manifold for the KSE at a domain size of $L=22$, which exhibits spatiotemporal chaotic dynamics. An example trajectory of this system is shown in Fig.~\ref{fig:Data_KSE_22_44_66_88-a}. This system, although formally infinite dimensional, has dynamics dictated by a nonlinearly embedded 8 dimensional manifold, as suggested by a variety of methodologies \citep{Ding2016,Takeuchi2011,Yang2009}. We show in Fig.~\ref{fig:SV_KSE_L22_L44_L66_L88-a} our method automatically learns an $\mathbb{R}^8$ latent space when trained over 40,000 ambient snapshots sampled on 64 spatial mesh points.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{Data_KSE_22_44_66_88}
        \captionsetup[subfigure]{labelformat=empty}
      	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:Data_KSE_22_44_66_88-a}\end{subfigure}
     	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:Data_KSE_22_44_66_88-b}\end{subfigure}
        \begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:Data_KSE_22_44_66_88-c}\end{subfigure}
     	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:Data_KSE_22_44_66_88-d}\end{subfigure}
		\caption[]{Typical velocity evolutions for the KSE in domain sizes of a) $L=22$, b) $L=44$, c) $L=66$, and d) $L=88$. \MDG{\sout{need to report mesh size -- we need many more grid points at higher $L$ values}}}
		\label{fig:Data_KSE}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{Drafting/SV_KSE_L22_L44_L66_L88}
        \captionsetup[subfigure]{labelformat=empty}
    	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:SV_KSE_L22_L44_L66_L88-a}\end{subfigure}
     	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:SV_KSE_L22_L44_L66_L88-b}\end{subfigure}
        \begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:SV_KSE_L22_L44_L66_L88-c}\end{subfigure}
     	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:SV_KSE_L22_L44_L66_L88-d}\end{subfigure}
		\caption[]{Singular values of learned latent spaces for the KSE a) $L=22$, b) $L=44$, c) $L=66$, and d) $L=88$.}
		\label{fig:SV_KSE_L22_L44_L66_L88}
	\end{center}
\end{figure}


For increasing domain sizes of of the KSE, the spatiotemporal dynamics of the system increases in complexity and chaoticity, shown in Fig.~\ref{fig:Data_KSE}. We extend our framework in Fig.~\ref{fig:SV_KSE_L22_L44_L66_L88} to these more complex KSE systems with domain sizes of $L=44, 66, 88$ sampled on a uniform spatial mesh of 64, 64, and 128 points, respectively. We highlight here that previous autoencoder methods \citep{Linot2020,Linot2021} struggle to make distinctions in the manifold dimension for these systems while our framework shows a clear boundary. Prior works relying on high-precision analyses of the governing equations have indicated that the manifold dimension for the KSE scales linearly with the domain length $L$ \citep{Yang2009,Takeuchi2011}. Here we show in Fig.~\ref{fig:SV_KSE_Scaling} we are able to recover this scaling without knowledge or analyses of the underlying governing equations.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.8\textwidth]{SV_KSE_Scaling}
		\caption[]{Manifold dimension estimates for $L=22, 44, 66, 88$. Each marker corresponds to the mean and standard deviation estimated by 5 randomly initialized models.}
		\label{fig:SV_KSE_Scaling}
	\end{center}
\end{figure}

For comparison, we show in Fig.~\ref{fig:MSVD_KSE_L22_L44-a} and Fig.~\ref{fig:MSVD_KSE_L22_L44-b} the MSVD applied to the same KSE datasets described above for domain sizes of $L=22, 44$, respectively. MSVD estimates $d_m$ by observing a separation in growing singular values as a function of sample neighborhood radius, $r$. We highlight here that the MSVD, given these datasets, is unable to distinctively identify $d_m=8, 18$. We comment this is likely due to limitations of MSVD requiring small enough $r$ neighborhoods to accurately capture the highly nonlinear manifold. Geometrically, if the manifold is not locally round, i.e. the manifold has various length scales, then at too large of $r$ these scales are not visible. However, in order to work in the limit of infinitesimally small scales, it would require our ensemble of data points to have neighboring points at very small $r$, which is generally not a luxury for data sampled from highly nonlinear systems. In our MSVD application, we were unable to traverse lower values of $r$ without encountering neighborless point cloud samples. Many complex dynamical systems do not uniformly populate their underlying manifolds, resulting in regions of high and low density. As a result, it is difficult to collect dynamical data in which the manifold is represented with uniform density or to collect enough data such that low probability regions are dense when natural occurrences these regions are low. We emphasize here that our presented framework was able to achieve an accurate estimate despite this local data limitation.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.8\textwidth]{MSVD_KSE_L22_L44}
        \captionsetup[subfigure]{labelformat=empty}
    	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:MSVD_KSE_L22_L44-a}\end{subfigure}
     	\begin{subfigure}[b]{0\textwidth}\caption{}\vspace{-10mm}\label{fig:MSVD_KSE_L22_L44-b}\end{subfigure}
		\caption[]{Performing Multiscale SVD on the KSE L=22, 44 dataset.}
		\label{fig:MSVD_KSE_L22_L44}
	\end{center}
\end{figure}


\subsubsection{Kolmogorov Flow $n=2, Re=14.4$}
Kolmogorov flow is a 2D flow described by the Navier-Stokes equations driven by a sinusoidal forcing term with wave number $n$. For $n=2$, the dynamics of the flow become chaotic at a $Re=14.4$. Here the ambient state space of vorticity, $\omega$, is represented by the $32\times32$ collocation points. The chaotic dynamics of this particular flow system are characterized by intermittent bursting events followed by quiescent periods. These events correspond to the system bursting in kinetic energy as it migrates between shadowing events of the relative periodic orbits embedded in the attractor. 

%\subsubsection{Kolmogorov Flow $n=2, Re=20.0$}
%mega chaotic

\subsubsection{Global manifold estimates vs local estimates: quasiperiodic dynamics on a 2-torus}
We now turn our attention to a particle in $\mathbb{R}^3$ traversing along the surface of a 2-torus with poloidal and toroidal speeds that lead to quasiperiodic dynamics, visualized in Fig.~\ref{fig:Data_Torus2D}. Given infinite time, the particle will densely cover the surface of the torus. Although this system lives on a two dimensional submanifold, a single global representation is not possible to obtain without discontinuities. Here we apply our framework to this dataset, which consists of snapshots of the particle's 3 spatial coordinates along a trajectory. In this example, we also use an overcomplete network design, $z\in\mathbb{R}^{10}$, to highlight that even when $d_z>d_n$, excess degrees of freedom are still correctly decayed. We show in Fig.~\ref{fig:SV_Torus2D} that when our framework is tasked with learning a global representation by training over the entire dataset, it obtains a 3-dimensional latent space. However, as described by \cite{FloryanCANDyMan2022}, the application of charts and atlases, i.e. the decomposition of the manifold into submanifolds, the intrinsic dimension of the data can be observed. In Fig.~\ref{fig:SV_Torus2D}, we show our method applied to the same dataset that has been divided into charts, illustrated in Fig.~\ref{fig:Data_Torus2D}. We show that for each subdomain, our method automatically learns a minimal 2-dimensional representation of the data while simultaneously discarding the remaining superfluous degrees of freedom.
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.90\textwidth]{Data_Torus2D_Global_Charts}
		\caption[]{Quasiperiodic dynamics along the surface of a torus a) global b) charted (local).}
		\label{fig:Data_Torus2D}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.90\textwidth]{SV_Torus_Combined}
		\caption[]{Singular values of learned latent spaces for the a) Global torus dataset and b) charted (local) torus dataset}
		\label{fig:SV_Torus2D}
	\end{center}
\end{figure}

\newpage

\subsection{A common manifold coordinate and a natural extension to reduced-order/state-space modeling/time-series forecasting}

We now turn our attention to the latent space learned by our framework. We emphasize here that typical autoencoders do not learn a common latent space in the absence of explicit constraints or novel architectural designs that is reproduceable between randomly initialized models. Shown in Fig.~XX is a visualization of the latent space encoding, $z_{vanilla}$, learned by two randomly initialized autoencoders trained over the KSE $L=22$ dataset. We note that the learned latent spaces are both full rank and importantly different. Shown in Fig.~XX is a visualization of the latent space encoding $h^{+}=U^Tz$ obtained from our framework, which exhibits a minimal $\mathbb{R}^8$ representation and importantly approximately identical modal evolutions up to a sign (i.e. the orthogonal bases are equivalent). Finally, in Fig.~XX, we show that this phenomenon is not a product of projecting the latent space onto its latent basis by projecting the latent space encoding shown in Fig.~XX onto its respective singular basis $h_{vanilla}^{+}=U_{vanilla}^T z_{vanilla}$.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{Latent_KSE}
		\caption[]{Example learned latent code space $z$ of (a),(b) vanilla autoencoders and (c),(d) our framework trained over KSE $L=22$ data. The same code space projected onto the respective singular vector bases, $h^{+}=U^Tz$, of (e),(f) vanilla autoencoders and (g),(h) our framework.}
		\label{fig:Latent_KSE}
	\end{center}
\end{figure}

As our framework automatically learns a rank-deficient representation $h^{+}$, the minimal representation can be isolated by simply truncating the singular basis vectors appropriately $UU^Tz\approx\hat{U}\hat{U}^Tz$ without loss of information, where $h^{+}=U^Tz$, $h=\hat{U}^Tz$, and $\hat{U}^T$ is equal to the first $d_m$ (identified via the singular value spectra) columns of $U$. Here $h$ is an approximately lossless and minimal representation describing the dynamics of the data. We can map ambient snapshots to this approximate manifold representation by simply extending our definitions of encoding and decoding to $h$,
\begin{equation}
    \begin{split}
        h & := \mathcal{E}_h(u;\theta_E,\theta_W,U) = \hat{U}^T \mathcal{W}(\mathcal{E}(u;\theta_E);\theta_W) \\
        \tilde{u} & := \mathcal{D}_h(h;\theta_D,U) = \mathcal{D}(\hat{U}h;\theta_D)
    \end{split}
\label{eq:encode_h}
\end{equation}
where $\mathcal{E}_h$ and $\mathcal{D}_h$ simply subsume the intermediate transformations required to map between $h$ and $u$. With our extended definitions of encoding and decoding, we now have 1) an estimate of $d_h$, 2) obtained the coordinate system $h$ parameterizing the manifold, and 3) have the explicit mapping functions $\mathcal{E}_h$ and $\mathcal{D}_h$. With access to these three, a natural application is state-space model and forecasting. We show a schematic of this extension in Fig.~\ref{fig:Schematic_Forecasting}.

We demonstrate this natural application using the KSE, where we train a Neural ODE, $\dot{h}=g(h;\theta_g)$, to model the dynamics in $h$ in time. Shown in Fig.~\ref{fig:Latent_KSE_Forecasting}, is an example trajectory from the KSE. For reference, shown in Fig.~\ref{fig:Latent_KSE_Forecasting} is the $\mathcal{E}_h$ encoded manifold representation of the same trajectory. From a single encoded  initial ambient state, we can perform the entire systems forecast in the manifold space. This forecasted trajectory is shown in Fig.~\ref{fig:Latent_KSE_Forecasting}. Naturally, the ambient representation of this trajectory can be completely recovered via $\mathcal{D}_h$, shown in Fig.~\ref{fig:Latent_KSE_Forecasting}.  We emphasize that because the KSE is a chaotic dynamical system, the ground truth and forecast will eventually diverge. However, despite this, the relevant time scale (Lyapunov time) of this system is $~20$ time units and we achieve good agreement on the order of this scale. From this, we highlight that our learned manifold coordinate system is conducive for forecast modeling and our mapping functions produce good ambient reconstruction. 

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{Schematic_Forecasting}
		\caption[]{Schematic for extending framework for forecasting in the manifold coordinate system.}
		\label{fig:Schematic_Forecasting}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{Latent_KSE_Forecasting}
		\caption[]{Example ground truth trajectory of the KSE in the a) ambient space and  b) the learned manifold coordinate representation. d) A time series forecast made using a Neural ODE in the d) manifold coordinate beginning from the same initial condition. c) The ambient space reconstruction decoded from the Neural ODE forecasted manifold trajectory.}
		\label{fig:Latent_KSE_Forecasting}
	\end{center}
\end{figure}


\newpage

\subsection{Extensions of current understandings and network learning dynamics}

\subsubsection{Rank Evolution and Gradient Tracing in a Nonlinear Network}

\begin{itemize}
\item rank of network weights vs. training
\item rank of gradient vs. training
\item rank of representation vs. training
\end{itemize}

We now turn our attention towards characterizing the learning dynamics of our $\lambda$-Implicit autoencoder in space (i.e. forward pass depth within the network) and time (i.e. increasing training episode) to pinpoint ``where" and ``when" the network achieves its low-rank representation.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.50\textwidth]{SV_KSE_L22_Dyn}
		\caption[]{Singular Values evolution during training}
		\label{fig:SV_KSE_L22_Dyn}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{track_rank_weights}
		\caption[]{Space-time tracking rank of the layer weights}
		\label{fig:track_rank_weights}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{track_rank_gradients}
		\caption[]{Space-time tracking the rank of the gradients}
		\label{fig:track_rank_gradients}
	\end{center}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{track_rank_representation}
		\caption[]{Space-time tracking the rank of the learned representation}
		\label{fig:track_rank_representation}
	\end{center}
\end{figure}
\newpage

\subsection{Robustness and Parameter Sensitivity}
\begin{itemize}
\item noise
\item over regularization via excess $\lambda$, excess $W$
\end{itemize}

\subsubsection{Dependence on weight decay, scaling for $\lambda$}
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_KSE_Learning_Dyn}
		\caption[]{Singular values of learned latent spaces for the KSE L=66}
		\label{fig:SV_KSE_Learning_Dyn}
	\end{center}
\end{figure}


\subsubsection{Dependence on $z\in\mathbb{R}^c$}
Currently appears you need $c>d_h$
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_KSE_c_values}
		\caption[]{Singular values of learned latent spaces for the KSE L=66}
		\label{fig:SV_KSE_c_values}
	\end{center}
\end{figure}
\subsubsection{Dependence on $L$}
Similar findings as \citep{Jing2020}. Weight sharing $L$ leads to worsened performance.

\newpage

\subsection{Implicit Presentation of a Manifold Interpretation}

Let $n$ be the ambient dimension such that $x\in\mathbb{R}^n$. Let $\mathcal{M}$ be a manifold of dimension $m$ embedded in $n$. The codimension is defined as $k=n-m$. The implicit representation of $\mathcal{M}$ is thus defined by placing $k$ level set constraints on points $\mathbb{R}^n$. We require that these $k$ constraints, $g_i(x)=0$ for $1\le i \le k$, to be $C^1$ and not trivially zero. Furthermore, we require that $\nabla g_i(x)$ be linearly independent on $\mathcal{M}$.

Special Case $z\in\mathbb{R}^{c=n}$: In this case there is no explicit dimensionality reduction, i.e. $\mathbb{R}^n \xrightarrow{E(x)}\mathbb{R}^n$. We define the mapping of $x$ to our final learned representation as $h=E(x)U\in\mathbb{R}^n$. In this representation, we know the singular values, i.e. variance, of $\mathcal{M}$ in each of the orthogonal directions of $h$, as $E(x)$ was trained and $U$ was computed from $x\in\mathcal{M}$. 

The singular values reveal that there are $m$ nonzero singular values and  $k$ ~zero singular values in our singular values. These $k$ zero singular values indicates that there is no variance in these directions--i.e. they are constant in our $h$ representation. Importantly, directions with no variance are equivalent to planar level sets. This reveals that the model learns $g_i(x)=y_{m+i}=E(x)U_{m+i}=0$ for $1 \le i \le k$. These $g_i(x)$ are the implicitly learned constraint functions that constrain $\mathcal{M}$ in $\mathbb{R}^{c=n}$ to $\mathbb{R}^m$. Thus the points on the manifold under these constraints in $h$ are defined by the subset $[y_1 ... y_m]$.

Returning to the previous requirements of our constraints we find that: $g_i(x)=E(x)U_{m+i}=0$ is $C^1$ as NNs are once differentiable, $\nabla g_i(x)=\nabla E(x)U_{m+i}$ are orthogonal to each other satisfying linear independence on $\mathcal{M}$, and $g_i(x)$ is not trivially zero.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{ImplicitManifold}
		\caption[]{Cartoon of Implicit Manifold Presentation}
		\label{fig:ImplicitManifold}
	\end{center}
\end{figure}

\newpage

% \subsection{Forecasting in Manifold Space}
% \begin{itemize}
% 	\setlength\itemsep{0pt}
% 	\setlength{\parskip}{0pt}
% 	\item Dynamics in $z$, highlight activation, truncation
% 	\item Forecasted Dynamics in latent space
% 	\item Reconstruction full space
% 	\item Learned Manifold space
% \end{itemize}
% \begin{figure}[H]
% 	\begin{center}
% 		\includegraphics[width=0.95\textwidth]{AL_Activated_Modes}
% 		\caption[]{Activated encoded modes of the Archemedean Lorenz}
% 		\label{fig:AL_Activated_Modes}
% 	\end{center}
% \end{figure}


\end{singlespace}

\newpage

\textbf{Chap 5 Manifold Notes:}
\begin{itemize}
	\setlength\itemsep{0pt}
	\setlength{\parskip}{0pt}
	\item manifolds each have a certain dimension $m$. This is a positive integer that tells us how many independent coordinates are needed to describe it (at least locally)
	\item e.g. Earth is a 2D manifold, locations are described by 2 quantities (latitude, longitude) locally. Note there is a discontinuity in longitude
	\item $m$-dimensional manifolds $M$ are subsets of the $n$-dimensional Euclidean space $\mathbb{R}^n$
	\item $m=0$ are isolated points
	\item $\mathbb{R}^n$ is the ambient space in which $M$ lies
	\item hypermanifolds have maximal dimension $n-1$
\end{itemize}

\newpage
\textbf{Appendix}
KURAMOTO-SIVASHINSKY L=44
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_KSE_L22_Combined}
		\caption[]{Singular values of learned latent spaces for the KSE L=22}
		\label{fig:SV_KSE_L22}
	\end{center}
\end{figure}
KURAMOTO-SIVASHINSKY L=44
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_KSE_L44_Combined}
		\caption[]{Singular values of learned latent spaces for the KSE L=44}
		\label{fig:SV_KSE_L44}
	\end{center}
\end{figure}

KURAMOTO-SIVASHINSKY L=66
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_KSE_L66_Combined}
		\caption[]{Singular values of learned latent spaces for the KSE L=66}
		\label{fig:SV_KSE_L66}
	\end{center}
\end{figure}

KURAMOTO-SIVASHINSKY L=88

Insert standard AE MSE plot for comparison

\subsubsection{The MNIST Handwriting Dataset}
MNIST explanation
\MDG{does the drift problem happen here? This might be a good example for discussing this, since it appeared in the original LeCun paper.}
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.95\textwidth]{SV_MNIST_Combined}
		\caption[]{Singular values of learned latent spaces for the MNIST Handwriting Dataset}
		\label{fig:SV_MNIST}
	\end{center}
\end{figure}
\newpage

==> abstract.tex <==
While many phenomena in physics and engineering are formally high-dimensional, the underlying dynamics that govern them often live on a lower-dimensional manifold. In this chapter, we introduce an autoencoder framework that combines implicit regularization with weight decay to automatically estimate the underlying dimensionality of the data, produce an ordered and orthogonal manifold coordinate system, and provide the mapping functions between the ambient space and manifold space, allowing for out-of-sample projections. We validate our framework's ability to estimate the manifold dimension for a series of dynamical datasets of varying complexities and compare to several state-of-the-art estimators. We dissect our framework in ``space'' and ``time'' to glean insight into the mechanism of low-rank learning and find that collectively each of the implicit regularizing layers compound the low-rank representation and even self-correct during training. We show that this framework can be naturally extended for applications of state-space modeling and forecasting by modeling a spatiotemporally chaotic partial differential equation using only the manifold coordinates. Finally, we demonstrate our framework is relatively robust to hyperparameter choices.

==> introduction.tex <==
\begin{singlespace*}
\textbf{Introduce datasets/systems of interest. What properties do they have and why do we care. Introduce concept of manifold}

Nonlinear, dissipative, partial differential equations (PDEs) are ubiquitous in describing phenomena throughout physics and engineering that display complex nonlinear behaviors, out-of-equilibrium dynamics, and even spatiotemporal chaos. Although these formally infinite-dimensional partial differential equations can be extremely high-dimensional in the ambient space, the long-time dynamics that describe these dissipative flows are known or suspected to collapse onto finite-dimensional invariant manifolds \citep{Teman1977}. These so called ``inertial manifolds'', $\mathcal{M}\subset\mathbb{R}^{d_n}$, are objects with dimension $d_m$ embedded in the ambient space $\mathbb{R}^{d_n}$, where often times $d_m<<d_n$. That is to say, in order to accurately describe the manifold, and thus the underlying dynamics of these systems, only $d_m$ independent ``coordinates'' are needed (at least locally).

Obtaining this minimal manifold coordinate description for these systems is ideal for a number of dynamical applications such as state-space identification, reduced-order modeling, and system interpretability, as well as many other down-stream tasks such as classification. However, estimating the underlying dimensionality and obtaining the manifold coordinate transformations is generally a nontrivial task. Given access only to the high dimensional ambient space of the system, the challenge becomes the following: 1) how does one determine $d_m$, 2) how does one determine a $\mathbb{R}^{d_m}$ coordinate system describing $\mathcal{M}$, and 3) how does one obtain the mapping functions $\mathcal{E}:\mathbb{R}^{d_n} \rightarrow\mathbb{R}^{d_m}$ and $\mathcal{D}:\mathbb{R}^{d_m}\rightarrow \mathbb{R}^{d_n}$. In the interest of identifying and modeling the underlying core dynamics of these systems, our primary tasks are to address these three challenges  using a single framework trained on high-dimensional ambient data alone.

\textbf{Introduce methodologies in identifying manifold}

The aforementioned three challenges have been tackled by an extensive variety of methodologies but we emphasize that rarely are all three challenges simultaneously addressed--often times only the first challenge of identifying the manifold dimension is accomplished. For complex dynamical systems, many of these methods developed in systems theory rely on high-precision analyses and access to the underlying equations. For example, \citep{Yang2009,Yang2012} estimated the manifold dimension of the Kuramoto-Sivashinsky equation for a range of parameters by using Covariant Lyapunov Vectors and monitoring when the Lyapunov spectrum of each system begins to rapidly fall. \citep{Ding2016} corroborated the manifold dimension of the KSE for $L=22$ via a Floquet mode approach applied to organized unstable periodic orbits identified in the system. Although these methods are ``physically'' rooted, they require high precision computations that for more complex systems such as the Navier-Stokes equations, are nontrivial or even intractable tasks. Furthermore, these methods are nonviable when only data is available and the governing equations are not known.

Towards more generalized and data-driven approaches, the task of estimating the number of degrees of freedom required to represent a set of data without loss of information has been explored in the fields of pattern recognition, information sciences, and machine learning. These methods produce estimates of $d_m$ (or some upperbound) either using global, local, or even pointwise analyses of the dataset. In this work, we will focus on global and local methods as our proposed framework operates in these regimes. 

Global approaches tackle this challenge in several ways. Global projection methods, such as Principal Component Analysis (PCA) [XXXX] and its variants (e.g. Sparse PCA [XXXX] and Bayesian PCA [XXXX]), optimize a subspace in which the projection of the data minimizes some projection error. These methods are useful in that not only are they computationally tractable, they also directly provide the mapping functions to the low dimensional representation. However, they generally overestimate $d_m$ as they are linear methods and cannot inherently deal with nonlinearity. Nonlinear PCA, or deep autoencoders in general, deal with nonlinearity using neural networks tasked with autoassociation [XXXX]. In applications toward complex dynamical systems, \citep{Linot2020} [VLACHAS] used undercomplete autoencoders to estimate the manifold dimension of the Kuramoto-Sivashinsky equation tracking the mean squared reconstruction error (MSE) as a function of the bottleneck size of the models. When the MSE significantly dropped, it signified that the minimum number of degrees of freedom needed to represent the system data was reached. However, a drawback of this type of approach is it requires training a parametric sweep of models. Furthermore, as system complexity and domain sizes were increased, this MSE drop becomes less and less obvious \citep{Linot2020}.

Other global methods rely on nearest neighbor searches and neighborhood graphs. 
[] and [] proposed data-driven state-space reconstruction methods to the reconstruct chaotic attractors from noisy time series. Notably, these methods incorporate the false-nearest-neighbor metric to determine an optimal embedding dimension on the fly. This however requires the combinatoric computation of euclidean distances between training data points for a range of embedding dimensions at each iteration of training, which is not ideal for systems of increasing complexity and dimensionality.

Other global methods include counting methods such as Box-Counting Estimations, Hausdorff Dimension Estimates, 


\textbf{Introduce Other Dimensionality Reduction Methods}
Several notable methods of dimensionality reduction utilize local computations. These include ISOMAP, LLE. These methods

Another local 

ALSO cite previous lorenz dim counting method.

\textbf{Low Ranking Driving Forces}
Our deep learning framework utilizes two low-rank driving forces. The first is known as implicit regularization, which is a phenomenon observed in gradient-based optimization of deep linear networks (i.e. multiple linear layers in series) leading to low-rank solutions \citep{Gunasekar2017}. Although a series of deep linear layers is functionally and expressively identical to a single linear layer, the learning dynamics are between the two are different. The mechanisms of this phenomenon is an ongoing area of research with primary focus in matrix \citep{Gunasekar2017} \citep{Arora2019} factorization, tensor factorization \citep{CohenRazin2020}, and regression problems \AddText{CITE}. Importantly, it has been observed that implicit regularization does not occur for unstructured data sets such as random noise \citep{Arora2019}, indicating that the phenomenon depends on the underlying structure of the data. Recently, implicit regularization has been extended to autoencoders to learn low rank representations, improving learning representations for image-based classification and generative performance by \citep{Jing2020}, whose observation form the foundation in this work.

\textbf{Introduce weight-decay:}
The second low-rank driving force is weight-decay. Weight-decay is a popular weight regularization mechanism in deep learning that forces the network to make trade-offs between the standard loss of the learning problem with properties of the weights of the network, $\theta$, 
\begin{equation}
\mathcal{L} = L + \dfrac{\lambda}{2}  {\left\lVert \theta \right\rVert}_p^2.
\label{eq:weight_decay}
\end{equation}
For example, $L_2$ regularization corresponds to emphasizing the network weights be small while $L_1$ regularization corresponds to promoting sparsity in the network weights. For linear models, these $L_1$ and $L_2$ weight-decay penalties are known as Lasso and Ridge regression.

Recently, Mousavi-Hosseini et al. proved that in two-layer neural-networks the first layer weights converge to the minimal principal subspace spanned by a target function only when online stochastic gradient descent (SGD) is combined with weight decay. They found that weight-decay allowed for SGD to avoid critical points outside the principal subspace. Here we demonstrate a similar synergistic result when weight-decay is combined with implicitly-regularized autoencoders. 

%Chen et al. \citep{Chen2021} demonstrated the advantage of unifying sparsity and low-rank representations in attention mechanisms. 

Here our aim is to demonstrate that implicit regularization combined with weight-decay in deep autoencoders can be used for datasets that possess an underlying finite dimensionality i.e. manifold, to 1) estimate the dimensionality of the underlying manifold, 2) obtain the coordinate system describing the manifold, and 3) obtain mapping functions to and from the manifold coordinate. We highlight that our framework provides an orthogonal manifold coordinates basis organized in order of importance by construction and does not require extensive parametric model sweeps as previous methods have done[Linot,Vlachas]--only a sufficient upper-bound guess of the manifold dimension is sufficient. Furthermore, we have empirically observed that our framework learns approximately consistent manifold coordinates between models. As a result, our method stands as a natural first step for data-driven reduced-order/state space modeling and many other downstream tasks. 

We apply our method to a zoo of datasets ranging from synthetic data sets to physical systems that exhibit complex spatiotemporal chaotic dynamics including the Lorenz system, the Kuramoto-Sivashinsky equation, and Kolmogorov flow. To understand the mechanisms of our framework, we isolate the origins of low-rank in our models in both ``space" and ``time" and under a dynamical systems theory lens, we glean insight into network learning and provide a rational for how implicit regularization and weight decay work achieve a synergistic effect. We highlight the learning dynamics of manifold coordinates and demonstrate how to model and forecast dynamics in the manifold coordinates. 

Think about journal?\MDG{Machine Learning: Science and Technology? Data-Centric Engineering?} 

Think about how to include derivation appendix \MDG{For case with weight-decay (L2 regularization, I think we can refer to the new arxiv handbook of convergence methods to say that GD should give convergence: \cite{Garrigos.2023.10.48550/arxiv.2301.11235}.  At least under the conditions we impose, I think that the objective function is ``strongly convex".  Without L2 reg it's not (thus the zero eigenvalues).} 

\end{singlespace*}
 
